The Computational Complexity of the Game of Set and its Theoretical Applications

The game of SET is a popular card game in which the objective is to form Sets using cards from a special deck. In this paper we study single- and multi-round variations of this game from the computational complexity point of view and establish interesting connections with other classical computational problems. Specifically, we first show that a natural generalization of the problem of finding a single Set, parameterized by the size of the sought Set is W-hard; our reduction applies also to a natural parameterization of Perfect Multi-Dimensional Matching, a result which may be of independent interest. Second, we observe that a version of the game where one seeks to find the largest possible number of disjoint Sets from a given set of cards is a special case of 3-Set Packing; we establish that this restriction remains NP-complete. Similarly, the version where one seeks to find the smallest number of disjoint Sets that overlap all possible Sets is shown to be NP-complete, through a close connection to the Independent Edge Dominating Set problem. Finally, we study a 2-player version of the game, for which we show a close connection to Arc Kayles, as well as fixed-parameter tractability when parameterized by the number of rounds played.

==> 2pset.tex <==
\subsection*{Omitted parts from Section \ref{sec:2pset}.}


\subsubsection*{Proof of Theorem \ref{thm:2p-FPT}.}\label{app::2p-FPT}
(\emph{\tpset\ parameterized by the number of allowed rounds $r$ is FPT}.)


\begin{proof}

First, observe that hypergraph $G$ where the game is played should have an edge
dominating set of size at most $r$ and thus a hitting set of size at most $3r$.
If there is no hitting set of size at most $3r$, simply reply no because it's
then impossible for the first player to end the game in $r$ moves.  Otherwise
we compute such a hitting set.  This can be done in FPT time 
%(latest improvement appears to be the result of 
\cite{wahlstrom2007algorithms}.
%that computes a 3-hitting set in $O(2.076^k)$ as it is suggested in the table race of the \href{http://fpt.wikidot.com/fpt-races}{FPT wiki}.)
Name the vertices of the hitting set $h_1, h_2, \ldots, h_s$, where $s$ is the 
size of the hitting set.

We can now reduce our problem to an ordered version of \node\ on an $r$-partite
graph. In this version the input is an undirected simple graph $G'(V,E)$ where
$V$ is partitioned into $r$ independent sets $V_1,\ldots,V_r$. The two players
alternate turns, and in turn $i$ the current player must select a vertex from
$V_i$ so that it has no edges to previously selected vertices.

We can construct $G'$ from $G$ as follows: for each hyperedge $e$ of $G$
construct $r$ vertices $e_1,\ldots,e_r$ in $G'$, such that $e_i\in V_i$ for all
$i$. If two hyperedges $e,f$ share an endpoint in $G$ connect the vertices
$e_i,f_j$ for all $i\neq j$. It is not hard to see that player 1 has a winning
strategy in the new game if and only if he has a winning strategy of length at
most $r$ in the original game.

We will say that a vertex $e_i$ of $G'$ has color $j$ when the hitting set
vertex $h_j$ is contained in the hyperedge $e$. Notice that all vertices of
$G'$ have some color, and none can have more than three. Also, for any pair of
colors $i,j$ there is at most one vertex in each partite set that has both
colors $i$ and $j$, since by the Set property any two vertices of the original
hypergraph have a unique third vertex with which they form a Set. Finally, note
that for each $i$ such that $ 1\le i \le s$, the vertices with color $i$ form an
$r$-partite complete subgraph in $G'$, since they all come from hyperedges that
contain $h_i$.

Partition the set $V_r$ into subsets such that each set contains vertices with
exactly the same colors. The subsets where vertices have two or three colors
have, as we argued, size 1. Consider now the subset of vertices
$S_{r,i}\subseteq V_r$ which have color $i$ only. We first have the following:

\begin{claim} \label{claim:degree}

A vertex $e_j\in V_j$, with $j\neq r$ and $e_j$ not having color $i$ can have
at most $2$ neighbors in $S_{r,i}$.  

\end{claim}

\begin{proof}

Suppose that $e_j$ has three distinct neighbors in $S_{r,i}$. Let the
hyperedges corresponding to these vertices be $\{h_i,u_1,v_1\},\
\{h_i,u_2,v_2\},\ \{h_i,u_3,v_3\}$. Notice that $h_i$ is the only hitting set
vertex in these sets, as $i$ is the only color of vertices in $S_{r,i}$. Now,
$e_j$ contains $h_j$ which is distinct from $h_i$ and all other vertices in
these sets. So, in order for $e_j$ to intersect all three of these sets, two of
them must share a common vertex other than $h_i$. But this contradicts the Set
property that any two elements have a unique third with which they form a Set.
\qed
\end{proof}

From Claim \ref{claim:degree} we now know that if $S_{r,i}$ contains at least
$2r$ vertices, then it will be possible to play it if and only if no vertex with
color $i$ is played in the first $r-1$ moves. Perform the following
transformation: delete all vertices of $S_{r,i}$ and replace them with a single
vertex that is connected to all vertices in other partite sets that have color
$i$.

The above reduction rule is safe. To see this, consider any play of the first
$r$ moves. If a vertex of color $i$ is used, no vertex from $S_{r,i}$ can be
used in the last move in both graphs. If color $i$ is not used, some vertex of
$S_{r,i}$ can be used in both graphs, and it is immaterial which will be played
since this is the last move.

Because of the above we can now assume that $|S_{r,i}|\le 2r$. Thus,
$|V_r|=O(r^2) $, because we have $s=O(r)$ sets $S_{r,i}$, as well as the single
vertices which may have a pair of colors.

We will now move on to the preceding partite sets using a similar argument. We
need the following definition: if two vertices $e_i,f_i$ of same color $c$ in the 
same partite set $V_i$ have exactly the same neighbors in all sets $V_j$ for $j>i$, then they
are called equivalent. We call such vertices equivalent because, if both
are available to be played at round $i$ they can be selected interchangeably
without affecting the rest of the game. Observe, that equivalent vertices have 
the same neighbors in $V_j$ for all $j\ge i+1$. Also observe that each equivalence
class cannot have more than $2$ neighbors. Namely, if two vertices of same color 
$c$ have at least one common neighbor then from claim \ref{claim:degree} this 
common neighbor cannot have more than these two vertices as common neighbors from 
color class $c$. On the other hand, if two or more vertices of color $c$ both have 
no neighbors, then we can all merge them into a single vertex. 


We will use this fact to show that we can reduce the graph so that in the end
$|V_i|\le |V_{i+1}|^{O(r)}$. 
Initially it may appear that the argument would lead to the conclusion
that $|V_i|\le 2^{|V_{i+1}|}$, since we have a different equivalence class of
each possible set of neighbors that a vertex of $V_i$ can have in $V_{i+1}$.
However, observe that each vertex of $V_i$ can have at most $2s$ neighbors with
which it does not share a color in $V_{i+1}$, since from Claim
\ref{claim:degree} it can have at most 2 neighbors in each group that
correspond to a different color. Thus, the possible neighborhoods are at most
${|V_{i+1}| \choose 2s} = |V_{i+1}|^{O(r)}$.

From the above it follows that the order of $G'$ after applying the above
preprocessing exhaustively is $2^{2^{O(r)}}$, which gives a kernel. \qed


\end{proof}


\subsubsection*{Proof of Corollary \ref{thm:arcfpt}.}\label{app:arcfpt}
(\emph{The natural parameterization of \arc\ by the number of rounds played is FPT.})

\begin{proof} 
(\emph{Sketch.} ) 
First, observe that graph $G$ where the game is played should have a vertex
cover of size at most $s=2r$. If not, reply no. The remaining vertices
forming an independent set can be divided into $2^{s}$ equivalence classes depending on
their neighbors in the vertex cover. 

If an equivalence class is large enough, playing any edge in an equivalence
class can be replaced by playing any other from the class without affecting the
rest of the game.  Namely, if an equivalence class is joined to $t$ vertices in
the vertex cover, there can be at most $t\leq s$ vertices played from this
class and it is unimportant which ones are played.  Thus, if a class has more
than $t$ vertices we can simply leave it with $t$ vertices and delete the rest.
 
Because of the above we have $2^s$ groups of vertices each containing at most
$s$ vertices and a vertex cover of size $s$. This means that the graph contains
at most $2^{2s}$ edges. Since in each turn a player selects an edge the number
of possible plays is at most $(2^{2s})^s = 2^{O(r^2)}$. Simply enumerating them
all gives an FPT algorithm. \qed

\end{proof}







